GENNI: Visualising the Geometry of Equivalences for Neural Network Identifiability

We propose an efficient algorithm to visualise symmetries in neural networks. Typically, models are defined with respect to a parameter space, where non-equal parameters can produce the same input-output map. Our proposed method, GENNI, allows us to efficiently identify parameters that are functionally equivalent and then visualise the subspace of the resulting equivalence class. By doing so, we are now able to better explore questions surrounding identifiability, with applications to optimisation and generalizability, for commonly used or newly developed neural network architectures.

==> old_text.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Meta-learning Background Text
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Meta-learning methodologies can be subdivided into three main sub-types: metric-based approaches \cite{matchingNets, prototypical, CAVIA}, model-based approaches \cite{santoro, hypernetworks, SNAIL} and optimization-based approaches \cite{MAML, reptile, CAVIA}. Metric-based approaches learn an embedding space where non-parametric nearest neighbors can be used for classification. Model-based approaches leverage the properties of specific model architectures, such as Recurrent Neural Networks, LSTMs  and memory augmented neural networks to learn how to update its or an external model's parameters. Optimization-based approaches frame the meta-learning problem as a bi-level optimization where the meta-objective is to learn meta-parameters $\theta$ suited for fast adaptation in a distribution of tasks by an optimization-based learning procedure such as gradient descent. Hybrid approaches have also been considered to combine the benefits of different approaches \cite{LEO, protomaml}.

Meta-learning methodologies can be subdivided into three main sub-types: metric-based approaches, model-based approaches and optimization-based approaches. Metric-based meta-learning methods aim to find ways to measure the similarity between the support and the query examples \cite {prototypical, siamese, matchingNets, relationnet, tadam}. Siamese networks \cite{siamese} constitute of two identical networks and work by extracting feature vectors from two examples, calculating the distance between the feature vector and convert it to a probability measure of being from the same class. Rather than comparing only two examples at a time, matching networks\cite{matchingNets} compare a query examples to a set of support examples after embedding them in a learnt feature space and classify the class of the query as that of its nearest neighbour. Prototypical networks \cite{prototypical} exploit intra-class variations by comparing the query examples to the mean feature embedding vector of each class from the support example instead of comparing to each support example. Relation network \cite{relationnet} provided an extension to the prototypical networks \cite{prototypical} where rather than learning an embedding to compare the data using Euclidean distance, both the  embedding function along with the similarity function are learnt.\\
\\
Optimization-based meta-learning approach meta-learning by designing or learning an optimization algorithm that can leverage the learnt information from the meta-training phase to adapt to the meta-testing stage \cite{MAML, reptile, CAVIA, iMAML, ravilstm}. An LSTM-based meta-learner \cite{ravilstm} was proposed that attempts to optimize another learner called a learner. MAML \cite{MAML} casts the meta-learning framework as a bi-level optimization, where the learning takes place over two nested loop. In the inner loop, the objective is to identify task-specific parameters while in the outer loop the objective is to learn general meta-parameters to aid the inner loop objective of a novel task. CAVIA \cite{CAVIA} addressed the meta-overfitting problem of MAML by partitioning the model's parameters into the task independent parameters and the context parameters. iMAML \cite{iMAML} derived a closed form solution of the inner loop optimization so that the outer loop optimization depends solely on the solution of the inner loop rather than the path taken from the inner loop optimization, tackling the computational inefficiency of meta-learning.\\
\\
Model-based meta-learning leverage the properties of specific model architectures, such as Recurrent Neural Networks, LSTMs  and memory augmented neural networks to learn how to update its or an external model's parameters \cite{santoro, SNAIL, metaNet, hypernetworks}. Memory augmented neural networks (MANN) \cite{santoro} were designed in order to provide provide two layers of learning, slow learning through gradual updates of their weights and fast learning through stored memory information. SNAIL \cite{SNAIL} combined the benefits of temporal convolutions with soft attention. Temporal convolutions allow the model to accumulate past experience while causal soft attention allows the model to focus on specific information from the whole context.












\section{Background}
\todo{Kate and Janith: DO THIS ASAP, you nonces}
\begin{enumerate}
    \item description of the identifiability problem; what have people looked at, how have they approached it?
    \item why is this a problem during optimisation?
    \item quotient spaces; what they do intuitively. How have they been visualised?
    \item mention motivation in transfer learning (reference Janith's work)

\end{enumerate}


\section{Preliminaries}
\subsection{Meta Learning}
The meta learning problem can be thought of as learning to learn. In conventional supervised machine learning, given a dataset of $n$ data points $\D := \{(x_1, y_1) ..., (x_n, y_n )\}$, we want to find a model $f_{\theta^*}$ such that 

\begin{equation} \label{eq:optimal_model}
    \theta^* = \argmin_{\Theta}{\L(\D, \theta; \phi)}.
\end{equation}
Here, $\Theta$ represents the parameter space of the models that we consider. That is, each model $f_\theta$ can be fully described by its parameter $\theta \in \Theta$. $\phi$  denotes the parameters of the learning method. These could include the choice of optimiser, the initialisation of the model parameters, and other hyperparameters. If the problem above is considered the learning problem for a particular task, then learning to learn would be the problem of finding suitable hyperparameters that are ideal for a class of \emph{related} tasks \cite{Hospedales2020}. 

Meta learning attempts to learn \emph{some structure} that is common amongst a set of related tasks such that learning a new task from that set is easier than learning it from scratch. A definition of \emph{relatedness} and \emph{a set of related tasks} is given in Section \ref{sec:relatedness}. Meta-learning methods often describe the full parameter space of the considered models as the product of \emph{global} parameters, and \emph{task-specific} parameters. Methods in transfer learning, few-shot learning and multi-task learning often can be classifed as applications of meta-learning.

Consider the few-shot meta-classification problem. Here, we there is a dataset $\D$ with a large number $N$ of data on a large number $K$ of classes. For each task $t$, we are given a smaller dataset $\D^t = \{(x_1, y_1), (x_n, y_n))\}_{n=1}^{N_t}$ where each input-output pair $(x_n, y_n)$ can be for one of $K^t < K$ classes and $N_t < N$; we must then find a classifier that $c_t$ such that a condition similar to Equation \ref{eq:optimal_model} is satisfied. During the meta-training phase, we are given datasets for several tasks; each dataset is split into training $\D^t_{tr}$ and validation $\D^t_{va}$ sets. The models are usually specified as 


\section{Notation}
We let $T$ denote a set of \emph{tasks} where a task is denoted by $t$, where the nature of $t$ will depend on the setting but should describe the task completely. A space of models is denoted by $\mc{M}$ which is parametrised by $\theta \in \Theta$. We assume that the parameter space can be written as the Cartesian product of outer and inner parameters (often called meta and inner parameters in the meta-learning literature) so that $\Theta = \Phi \times \Psi$ and $\theta = (\phi, \psi)$. Of note is the difference between the parameter space and function space; $\Phi \times \Psi$ and $\mc{M}_{\Phi} \times \mc{M}_{\Psi}$ where the first is typically a vector space while the second is not.

\section{Theoretical justification for current methods}
\subsection{The learning problem}
We begin by stating some definitions.

\begin{definition}
[Learning task]
A learning task is a target function $t: X \rightarrow Y$ which is the core \emph{learnable} component of a ML problem.
\end{definition}
It should be noted that a task here is usually any machine learning problem. This is immediately clear with supervised learning, since the $t$ in the definition is the data generating function. In unsupervised learning, we want to learn a map from the data to the structural components we are considering. For example, in k-means clustering, we learn a map from the data space to the corresponding cluster space; that is, each data point is mapped to its appropriate cluster. In reinforcement learning, a policy, which often maps from the state space to the action space is learned. In general, the learning task doesn't correspond to the data generating function or distribution; it is a map that is a part of ML problem that we can control, and learn. 

\begin{definition}
[Task space]
A space $\T$, where a learning task $t$ is an element of, is called the Task space. 
\end{definition}

\begin{definition}
[Model weight space]
The $d-$dimensional model weight space is $\Theta = \R^d$.
\end{definition}

\begin{definition}
[Model architecture]
Given a model weight space $\Theta$, the model architecture is a map $f: \Theta \times X \rightarrow Y$
\end{definition}

The model weight space gives us the parameter space of some model architecture. For each $\theta \in \Theta$, a model $f_\theta: X \rightarrow Y$ is given. For example, consider a linear model $f_\theta(x) = \theta^Tg(x)$, for $\theta \in \Theta$. In this case, each model $f_\theta$ is unique; that is $(\theta_1 \in \Theta) \neq (\theta_2 \in \Theta) \implies f_{\theta_1} \neq f_{\theta_2}$. In general however, this is not true. 

Consider now the model architecture given by $f_{\sin}(\theta, x) = f_{a, b}(x) = a\sin(x+b)$ for $((a, b) = \theta) \in (\Theta = \R^2)$. In the first parameter $a$, the situation is as the linear case; for any $a \in \R$ and for a fixed $b \in \R$, the model is uniquely identified. However, due to the periodic nature of the sine function, models repeat themselves as we vary along $b$. For example, $f_{a, 0}(x) = a\sin(x) = a\sin(x + 2\pi) = f_{a, 2\pi}$; in general, we can say that $f_{a, b} = f_{a, b+n\pi}$  $\forall n \in \Z$. Thus, we define the \emph{model space} to be as follows. 

\begin{definition}
[Model space] 
Given a model weight space $\Theta$ and a model architecture $f$, we can define an equivalence relation $\sim_m$ by 
\begin{equation} \label{eq:function_equivalence}
    (\theta_1 \in \Theta) \sim_m (\theta_2 \in \Theta) \iff f_{\theta_1}(x) = f_{\theta_2}(x) \quad \forall x \in X.   
\end{equation}
The quotient space $\Model = \Theta/_{\sim_m}$ is called the Model space.
\end{definition}

The model space gives us a way of bringing together all the model weights that are functionally the same w.r.t to the model architecture. We stated previously that the model weight space is Euclidean; the model space however, in general, have to be. In the case of linear models, the model weight space and model space are isomorphic, and the latter is therefore Euclidean. However, in the case of $f_{\sin}$ the model space is isomorphic to the cylinder $C^1 = \R \times \Circle^1$.

In ML, we want to find the element in the model space that best represents the task. We evaluate how well each model represents a tasks using the loss function.

\begin{definition}
[Loss function]
Given a task space $\T$ and a model space $\Model$, a map $l: \T \times \Model \rightarrow \R^+$ is called the loss function.
\end{definition}

The loss function measures a notion of distance between the task and a model. The learning algorithm uses the loss function to then find the best model for the given task; the learning algorithm can only distinguish between 2 models using the loss function. In the same way that 2 weights can correspond to the same function under the equivalence relation given in Equation \ref{eq:function_equivalence}, it is possible for 2 distinct models in $\Model$ to have the loss value. As far as the learning algorithm is concerned, these models are the same. Thus, we can defined a further quotient space. 

\begin{definition}
[Loss-wise identifiable model space]
Given a task $t \in \T$, a model space $\Model$ and a loss function $l$, we can define an equivalence relation $\sim_l$ on $\Model$ by 
\begin{equation} \label{eq:loss_equivalence}
    (m \in \Model) \sim_l (n \in \Model) \iff l(t, m) = \l(t, n).
\end{equation}
The quotient space $\Model_l = \Model/_{\sim_l}$ is called the Loss-wise identifiable model space.
\end{definition}

\subsection{Relatedness, Foliations and Transfer Learning} \label{sec:relatedness}
We begin once more by stating some definitions. 

\begin{definition}[$\Pi$-Relatedness]
Given a set of tasks $T$ and a transformation group $\Pi$ whose elements can act on $T$, two tasks, $t, s \in T$ are said to be $\Pi$-\emph{related} or just related to each other iff $\exists \pi_{ts} \in \Pi$, where $\pi_{ts}(t) = s$ and $\pi_{ts}^{-1}(s) = t$.
\end{definition}

This is distinct from similarity. Similarity is a geometric notion, while relatedness is a transformative notion.  

%I don't think similarity is needed here 
\begin{definition}[$\epsilon$-Similarity]
Given a set of tasks $T$, a metric $\rho$ on $T$, and some number $\epsilon \in \mathbb{R}^+$, two tasks $t, s \in T$ are $\epsilon$-\emph{similar} or just similar to each other with respect to $\rho$ if $\rho(t, s) < \epsilon$.
\end{definition}

The distinction between relatedness and similarity can be seen in Figure \ref{fig:related_vs_similar}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.32\textwidth]{figures/related_vs_similar}
    \caption{The distinction between similarity and relatedness. Similarity is defined in terms of an $\epsilon$-ball around a particular element. Here, points $t_2$ and $t_3$ are similar to $t_1$. On the other hand, relatedness is defined in terms of a transformation set; this relationship is shown as a line joining them. Thus, tasks $t_1, t_2$ and $t_3$ are related to each other. However, $t_4$ is not related to $t_2$ and $t_1$ though they are similar; $t_3$ is not similar to $t_2$ and $t_1$, though they are related.}
    \label{fig:related_vs_similar}
\end{figure}

The notion of relatedness depends on the transformation group that is chosen. The transformation group partitions the space of tasks $T$ into equivalence classes. The orbits of the transformation group will be called \emph{sets of related tasks}. 
\begin{definition}[Set of related tasks]
Given a set of tasks $T$ and a transformation group $\Pi$ w.r.t which a notion of relatedness is defined on $T$, the orbit defined by $\orbit_t := \{\pi(t) \: | \: \forall \pi \in \Pi\}$ is called the \emph{set of related tasks}.
\end{definition}

Each set of related tasks contains all tasks that are related w.r.t to $\Pi$. These sets define equivalence classes w.r.t the relation given by the chosen notion of relatedness. These equivalence classes are then a partitioning of $T$ into parallel spaces. This is shown in Figure \ref{fig:tessellation}. Such a structure can be described mathematically using foliations. 

\begin{figure} 
    \centering
    \includegraphics[width=0.7\textwidth]{figures/tessellation}

    \caption{The difference between a tessellation and parallel spaces. The shaded regions denote the subsets we are considering in each case. A tessellation creates disjoint, smaller subsets that are of the same dimension as the original set. Parallel spaces on the other hand creates disjoint subsets that are of a lower dimension than the original set.}
    \label{fig:tessellation}
\end{figure}

\subsection{Relation to existing work}
\paragraph{Prototypical networks} are a simple and intuitive method of solving the meta learning problem \cite{Snell2017}. This method is applied specifically to the meta-classification problem. The model is as follows.

The key intuition is that each class can be represented by a \emph{prototype} vector in some embedding space. The embeddings of each input in this space, for a particular class will be geometrically \emph{close} to its prototype. The embedding is given by $f_\theta: X \rightarrow C$, where $X$ is the input space, and $C$ is the embedding space. Given $\D_t^{tr}$ and $\D_t^{va}$, the prototype $c_k$ can be found by
\begin{equation}
    c_k = \frac{1}{N_{t,k}}\sum_{i}^{N_{t, k}}{f_\theta(x_i}),
\end{equation}
where $N_{t,k}$ is the number of data points of each class $k$ in the $\D_t^{tr}$, and $x_i$ is the first variable from the pair $(x_i, y_i) \in \D_t^{tr}$. Given a new test input $x$, the distribution over which classes it can be is given by
\begin{equation} \label{eq:prototypical_softmax}
    p(y=k|x) = \frac{\exp(-d(f_\theta(x), c_k))}{\sum_{k^{'}}\exp(-d(f_\theta(x), c_{k^{'}}))},
\end{equation}
where $d: C \times C \rightarrow \R^+$ is a metric on the embedding space. Equation \ref{eq:prototypical_softmax} is a softmax over the distances to the prototypes. 

The collection of all prototypes can be seen as the task specific parameters. The space $C^k = C_1 \times C_2 \times ... \times C_k = \R^k$ then is the space of all tasks that are possible within this set of related tasks. The full model then is specified by $\Theta \times C^k$; in the meta-training phase, we learn the best $\theta \in \Theta$ that best describes the set of related tasks we are given. Then we fix this, and adapt to new tasks by finding their prototypes. The mechanism for finding these is fixed in \cite{Snell2017}; there is no inner loop. 

Thus, we can see that this method has a notion of global and task specific parameters, and fits into the foliated view in this way. 

\subsection{Questions that can be asked}
\subsubsection{Does a new task belong to a particular set of related tasks?}
\paragraph{Question}
Suppose that we choose some model space. The meta-configuration of this model is then given by a chosen foliation. That is, the foliation specifies how we rectify the model space into global and task-specific parameters. Using these, we then meta a model for a set of tasks. We assume that these tasks are related. Typically, given a new task, we would assume that it is in the same set of related tasks, and attempt to adapt the model to it. That is, we would assume that the global parameters are fixed, and retrain the task-specific parameters. How good is the assumption that the new task belongs to the set of related tasks from the training phase? Can we, without having to \emph{train} the model, use the given data, identify how much it belongs to the previous set?

\paragraph{Possible answers}
\begin{itemize}
    \item Assuming that we fix the global parameters, we can evaluate a gradient of the loss function from the dataset of the new task. How different is the direction of this vector from the tangent space at the point of evaluation? That is, does the loss function direct the flow along the leaf given by the set of related tasks? 
    
   The argument here is that if the task does belong on the set of related tasks, then it should belong on the same leaf. If we were to begin on correct the leaf, then we would expect that the flow would, on average, be along the leaf. Maybe there is some analysis that can be done by restricting the loss function to the leaf. How does this compare to the full loss function? How does the difference between the parameter space and the function space of the model affect this? See the example about the sinusoid below. 

    \item The above was a first order test. We could try a zero-order test where we just evaluate the loss function at some random points (within some epsilon) on the same leaf, from the existing solutions. How good is the performance on average?
\end{itemize}


\subsection{Suggested experiments by theoreticians}
\input{experiments}

\subsection{Simple informative examples}
\paragraph{Least Squares.}
The simplest case we consider is that of meta-learning where each task is an instance linear regression. For each task $t$ there is a distribution $\mu$ which generates the data and write $D \sim \mu^n$ to mean that $D = (x_i, y_i)_{i=1}^n$ where each datapair is sampled iid from $\mu$ and the loss is the least squared loss and $x \in \R^{d}, y \in \R$. We assume that the true functional relationship for each task $t$ is given by a linear function, such that we can split $x = (x_{\phi}, x_{\psi})^{T} \in \R^{d_{\phi} + d_{\psi}}$ representing the global and local relationships of the data. The true function is thus given by
\begin{equation} 
    f^t(x) = \theta^{T}x = \phi^{T}x_{\phi} + \psi^{T}x_{\psi}.
\end{equation}
note that here $\phi$ is independent of $t$ since it's global while $\psi$ will change depending on task by assumption of the framework.

In this setting the two sets $\mc{M}_{\Phi} \times \mc{M}_{\Psi}$ and $\Phi \times \Psi$ are isomorphic to each other and we can use the weights $(\phi, \psi)$ to represent functions directly. The diagram of this would be that of a "line" $\R^{d_{\phi}}$ with each point of this line having an orthogonal "line" representing the space $\R^{d_{\psi}}$ \todo{Make trivial foliation figure of space $\mc{M}_{\Phi} \times \mc{M}_{\Psi} = \R^{d_{\phi}} \times \R^{d_{\psi}}$}.

\paragraph{Generalised Least Squares.}
A slight generalisation of this is that of dictionary learning, where instead of using $x = (x_{\phi}, x_{\psi})^{T}$ we define a feature map of $\varphi: \R^d \to \R^F$ where again $F = d_{\phi} + d_{\psi}$ so that we use $\varphi(x)$ in place of $x$ in the least squares setting. This allows us to consider cases where combination of entries in a datapoint $x$ are both in the local and global relationships. In this case we have the functional form for a task to be
\begin{equation}
    f^t(x) =  \phi^{T}\varphi(x)_{\phi} + \psi^{T}\varphi(x)_{\psi}.
\end{equation}

As in the previous setting the function and weight space are isomorphic to each other.

\paragraph{Kernel Linear Regression.}
The most general setting for linear regression in the foliation framework is when we consider $\mc{M}_{\Phi} \times \mc{M}_{\Psi} = \mc{H}_{\Phi} \times \mc{H}_{\Psi}$ where $\mc{H}_{\Phi}, \mc{H}_{\Psi}$ are two arbitrary RKHS's. In this case we have two feature maps $\varphi_{\phi}, \varphi_{\psi}$ which maps to potentially infinite-dimensional RKHS's which are spaces of functions. This also means that the weights in this case will be a pair of functions $\theta = (\phi, \psi) \in \mc{H}_{\Phi} \times \mc{H}_{\Psi}$ and the true function for a task looks like
\begin{equation}
    f^t(x) = \scal{\phi}{\varphi_{\phi}(x)}_{\mc{H}_{\Phi}} + \scal{\psi}{\varphi_{\psi}(x)}_{\mc{H}_{\Psi}}
\end{equation}
An alternative view is that the feature maps in this case is a basis for the space, specifically they may be an orthonormal system. This means that we can view a function $f$ as a Generalised Fourier Series, $f = \sum_{i=1}^{\infty} f_i \varphi_i$ where $f_i = \scal{f}{\varphi_i}_{\mc{H}}$ and $\varphi_i$ is a base vector for the space $\mc{H}$. This would allow us to for example approximate a function through a truncated Fourier series by approximating $f = \sum_{i=1}^{\infty}f_i e_i \approx \sum_{i=1}^{T}f_i e_i$ which allows us to be in the finite vector case which will be simpler to simulate. \todo{clean up section, a lot of things are glossed over and does not necessarily follow convention of e.g. Fourier series with indices, domain of function and what not}

\subsection{Learning a Sinusoidal}
Assume that the function space where all of the true functions live in are of the form $\mc{F} = \{A \cos(x + b) \: | \: A \in \R^{+}, b \in [0, 2\pi)\}$. Arbitrarily we assume that $A = \phi$ and $b = \psi$ so that we are learning the global parameter $A$ which is shared by all tasks (all tasks have functions of the same amplitude) but each task has a different phase. In this case the weight space can be shown to $\Phi \times \Psi \cong \R^{+} \times \S^{1}$, but it also highlights the difference between the weight and function spaces; addition is readily defined for weights as $(A_1, b_1) + (A_2, b_2) = (A_1 + A_2, b_1 + b_2)$ which is in the space (for phase addition is modulo $2\pi$). However if we add these functions together we get 
\begin{align*}
    A_1 \cos(x + b_1) + A_2 \cos(x + b_2)
    & =  A_1 (\cos(x)\cos(b_1) - \sin(x)\sin(b_1) \\
    & \quad + A_2 (\cos(x)\cos(b_2) - \sin(x)\sin(b_2) \\
    & = (A_1\cos(b_1) + A_2\cos(b_2))\cos(x) \\
    & \quad - (A_1\sin(b_1) + A_2\sin(b_2))\sin(x) 
\end{align*}
which is not in the function space.

\section{Optimization Notes}

\input{optimization_notes}







% \section{Theory} \label{sec:theory}
% \todo{Janith, Daniel}

% \begin{enumerate}
%     \item How does this relate to geometry?
%     \item Can move definitions to appendix! Focus on just making sure we have all the ones needed!
% \end{enumerate}

% We let $T$ denote a set of \emph{tasks} where a task is denoted by $t$, where the nature of $t$ will depend on the setting but should describe the task completely. A space of models is denoted by $\mc{M}$ which is parameterised by $\theta \in \Theta$. We assume that the parameter space can be written as the Cartesian product of outer and inner parameters (often called meta and inner parameters in the meta-learning literature) so that $\Theta = \Phi \times \Psi$ and $\theta = (\phi, \psi)$. Of note is the difference between the parameter space and function space; $\Phi \times \Psi$ and $\mc{M}_{\Phi} \times \mc{M}_{\Psi}$ where the first is typically a vector space while the second is not.

% \begin{definition}
% [Learning task]
% A learning task is a target function $t: X \rightarrow Y$ which is the core \emph{learnable} component of a ML problem.
% \end{definition}
% It should be noted that a task here is usually any machine learning problem. This is immediately clear with supervised learning, since the $t$ in the definition is the data generating function. In unsupervised learning, we want to learn a map from the data to the structural components we are considering. For example, in k-means clustering, we learn a map from the data space to the corresponding cluster space; that is, each data point is mapped to its appropriate cluster. In reinforcement learning, a policy, which often maps from the state space to the action space is learned. In general, the learning task doesn't correspond to the data generating function or distribution; it is a map that is a part of ML problem that we can control, and learn. 

% \begin{definition}
% [Task space]
% A space $\T$, where a learning task $t$ is an element of, is called the Task space. 
% \end{definition}

% \begin{enumerate}
%     \item We define the parameter space and function space. We do not need to worry about tasks.
%     \item Define a model/network/architecture. What is needed for that. Domain, Codomain and parameter space. \item The parameter space has the standard topology and we would like to understand the quotient toplogy under the equivalence relation given by the model architecture. 
%     \item Understanding the model architecture has been difficult so we would like to understand only the properties related to an equivalence class. 
% \end{enumerate}

% The properties of an equivalence class we would like to understand better:
% \begin{enumerate}
%     \item Connectedness, scaling symmetries. Maybe give examples here? This could lead naturally to our method to understad it better. Janith? 
% \end{enumerate}

% \begin{definition}
% [Model weight space]
% The $d-$dimensional model weight space is $\Theta = \R^d$.
% \end{definition}

% \begin{definition}
% [Model architecture]
% Given a model weight space $\Theta$, the model architecture is a map $f: \Theta \times X \rightarrow Y$
% \end{definition}

% The model weight space gives us the parameter space of some model architecture. For each $\theta \in \Theta$, a model $f_\theta: X \rightarrow Y$ is given. For example, consider a linear model $f_\theta(x) = \theta^Tg(x)$, for $\theta \in \Theta$. In this case, each model $f_\theta$ is unique; that is $(\theta_1 \in \Theta) \neq (\theta_2 \in \Theta) \implies f_{\theta_1} \neq f_{\theta_2}$. In general however, this is not true. 

% Consider now the model architecture given by $f_{\sin}(\theta, x) = f_{a, b}(x) = a\sin(x+b)$ for $((a, b) = \theta) \in (\Theta = \R^2)$. In the first parameter $a$, the situation is as the linear case; for any $a \in \R$ and for a fixed $b \in \R$, the model is uniquely identified. However, due to the periodic nature of the sine function, models repeat themselves as we vary along $b$. For example, $f_{a, 0}(x) = a\sin(x) = a\sin(x + 2\pi) = f_{a, 2\pi}$; in general, we can say that $f_{a, b} = f_{a, b+n\pi}$  $\forall n \in \Z$. Thus, we define the \emph{model space} to be as follows. 

% \begin{definition}
% [Model space] 
% Given a model weight space $\Theta$ and a model architecture $f$, we can define an equivalence relation $\sim_m$ by 
% \begin{equation} \label{eq:function_equivalence}
%     (\theta_1 \in \Theta) \sim_m (\theta_2 \in \Theta) \iff f_{\theta_1}(x) = f_{\theta_2}(x) \quad \forall x \in X.   
% \end{equation}
% The quotient space $\Model = \Theta/_{\sim_m}$ is called the Model space.
% \end{definition}

% The model space gives us a way of bringing together all the model weights that are functionally the same w.r.t to the model architecture. We stated previously that the model weight space is Euclidean; the model space however, in general, have to be. In the case of linear models, the model weight space and model space are isomorphic, and the latter is therefore Euclidean. However, in the case of $f_{\sin}$ the model space is isomorphic to the cylinder $C^1 = \R \times \Circle^1$.

% In ML, we want to find the element in the model space that best represents the task. We evaluate how well each model represents a tasks using the loss function.

% \begin{definition}
% [Loss function]
% Given a task space $\T$ and a model space $\Model$, a map $l: \T \times \Model \rightarrow \R^+$ is called the loss function.
% \end{definition}

% The loss function measures a notion of distance between the task and a model. The learning algorithm uses the loss function to then find the best model for the given task; the learning algorithm can only distinguish between 2 models using the loss function. In the same way that 2 weights can correspond to the same function under the equivalence relation given in Equation \ref{eq:function_equivalence}, it is possible for 2 distinct models in $\Model$ to have the loss value. As far as the learning algorithm is concerned, these models are the same. Thus, we can defined a further quotient space. 

% \begin{definition}
% [Loss-wise identifiable model space]
% Given a task $t \in \T$, a model space $\Model$ and a loss function $l$, we can define an equivalence relation $\sim_l$ on $\Model$ by 
% \begin{equation} \label{eq:loss_equivalence}
%     (m \in \Model) \sim_l (n \in \Model) \iff l(t, m) = \l(t, n).
% \end{equation}
% The quotient space $\Model_l = \Model/_{\sim_l}$ is called the Loss-wise identifiable model space.
% \end{definition}

% \section{Visualisation Algorithm} \label{sec:method}
% \todo{Daniel, and Isak}
% When we parameterise the model space $\mc{M}$ by a model architecture $f$ and a model weight space $\Theta$, for any function in $\mc{M}$ we often have several weights leading to the same function. This is particular common in neural networks architectures which introduce symmetries [cite work on this here] or invariances due to the activation function [cite work on this here]. The map from a function $g \in \mc{M}$ to the set of weights $\Theta_g = \{\theta \in \Theta | f_{\theta} = g\} $ is called the quotient map in topology. In this section we develop an algorithm for approximating this quotient map by assigning weights on a grid to bins representing approximate equivalence classes. Let $\Theta_D \subseteq \Theta$ be a discretisation of the space $\Theta$. Since $\Theta_D$ is finite we index it as $\Theta_D = (\theta_i)_{i=1}^n$. We will search over $\Theta_D$ to find weights which represents similar functions, we define this below.

% By properties of the norm, two functions $f, g$ on a compact domain $X$ being equal is the same as $\norm{f - g} = 0$. We let the norm be the normalised L2 norm, $\norm{f}^2 = \int_X f(x)^2 \dl x$ and for a set $C \subseteq X$ we let $\norm{f}_{C}$ be the norm of the functions restricted to $C$, $\norm{f}^2_C = \int_C f(x)^2 \dl x$. We define an $\epsilon$-equivalence class on $C$ to be the set of weights $\{\theta_{1}, \theta_2 \in \Theta_D | \norm{f_{\theta_1} - f_{\theta_2}}_C \leq \epsilon\}$. We note that this is not a true partition of $\Theta_D$ since we lost transitivity as we can have $\theta_1, \theta_2, \theta_3$ with $\norm{f_{\theta_1} - f_{\theta_2}}_C \leq \epsilon$ and $\norm{f_{\theta_2} - f_{\theta_3}}_C \leq \epsilon$ but  $\norm{f_{\theta_1} - f_{\theta_3}}_C > \epsilon$ in addition to the $\epsilon$-equivalence classes not necessarily being disjoint as they can overlap. Still we believe, and show in later sections, that this approximation captures what we mean by weights leading to the same function well enough in practice. We let $B$ denote the list of approximate equivalence classes and at the start of the algorithm it consists of $n$ approximate equivalence classes, each having just one element $b_i = \{\theta_i\}$.

% In practice we let $C$ be discrete, which means that $\norm{f - g}_C \leq \epsilon$ does not ensure that $\norm{f - g}$ is small in general. To answer questions like these we would need to use tools from Numerical Integration, in particular (Quasi)-Monte-Carlo [Cite] or Quadrature [Cite] analysis seems fruitful. We leave this analysis to the future.

% \begin{algorithm}
%     \caption{Calculate $\epsilon$-equivalence classes of $\Theta_D$}
%     \label{alg:eps-equiv-partition}
%     \begin{algorithmic}[1]
%         \Procedure{Eps-Equivalence-Binning}{$f, \Theta_D, C, \epsilon$}
%             \State $B \gets (b_1, \dots, b_n)$ \Comment{Initialise set of $\epsilon$-equivalence classes}
%             \For{$i = 1, \dots, n$}
%                 \For{$j = 1, \dots, n$}
%                     \If{$\norm{f_{\theta_i} - f_{\theta_j}}_C \leq \epsilon$} $b_i \gets b_i \cup \{\theta_j\}$
%                     \EndIf
%                 \EndFor
%             \EndFor
%             \State \textbf{return} $B$
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}
% Since $\epsilon$-approximate equivalence is reflexive we see that if we add $\theta_j$ to $b_i$ then also $\theta_i$ will be added to $b_j$. This means that we can prune the resulting set $B$ by removing any duplicates $b \in B$. The complexity of this algorithm is $O(n^2)$ as a function of $n$.

% [Speedup citation, KDTrees \url{https://arxiv.org/pdf/1301.3877.pdf}]

% This algorithm does not scale to higher dimensions, we propose to instead use an algorithm inspired by MCMC methods. For each $\theta_i$ we generate $m$ different starting points, $(\theta_{i, j})_{j=1}^M$ according to some sampling scheme. We use a gaussian distribution $\mc{N}(0, \sigma^2 I)$ and some discretisation $C$. For each $\theta_j$ we run stochastic gradient descent (SGD) on the objective $J(\theta) = \sum_{x \in C} (f_{\theta_i}(x) - f_{\theta}(x))^2$ starting from the different starting points generated previously, leading to the SGD outputs $(\tilde{\theta}_{i, j})_{j=1}^m$. We add the resulting $m$ weights to the $\epsilon$-equivalence class of $\theta_0$ as long as $\norm{f_{\theta_i} - f_{\tilde{\theta}_{i, j}}} \leq \epsilon$.

% \begin{algorithm}
%     \caption{Calculate $\epsilon$-equivalence classes of $\Theta_D$ (Gradient Descent)}
%     \label{alg:eps-equiv-partition-gd}
%     \begin{algorithmic}[1]
%         \Procedure{Eps-Equivalence-Binning}{$f, \Theta_D, C, \epsilon$}
%             \State $B \gets (b_1, \dots, b_n)$ \Comment{Initialise set of $\epsilon$-equivalence classes}
%             \For{$i = 1, \dots, n$}
%                 \State{Generate $m$ starting points $S \gets (\theta_{i, j})_{j=1}^m$}
%                 \For{$j = 1, \dots, m$}
%                     \State{$\tilde{\theta}_{i, j} \gets \text{SGD}(\theta_{i, j})$}
%                     \If{$\norm{f_{\theta_i} - f_{\tilde{\theta}_{i, j}}}_C \leq \epsilon$} $b_i \gets b_i \cup \{\theta_j\}$
%                     \EndIf
%                 \EndFor
%             \EndFor
%             \State \textbf{return} $B$
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

% \begin{itemize}
%     \item Algorithm / pseudo code
%     \item Optimisation
%     \item Discussion of complexity, etc
% \end{itemize}

==> outline.tex <==
We are going to go for "Visualization methods for manifolds"

\begin{enumerate}
    \item Basic Motivation: We will describe the function manifold which we would like to visualize. 
    \item Why: 
\end{enumerate}

Sections
\begin{enumerate}
    \item Intro: Background Motivation Definition (of manifold and everything). 
    \item Our method which we use: Describe the method we are using to prune. Basic results
    \item The Quotient space: AK's visualization + maybe Michalis (immediate next section)
    \item Further Applications and why this should be used: Generalization + Meta Learning + Interpretability
    \item Done
\end{enumerate}

\begin{definition}
    We define the manifold $\mathcal{F}$ defined by an architecture. Each function on the function manifold maps to various weights in the weightspace $\Theta$. 
\end{definition}


Janith: 
Write up the function manifold. 
What is the chart? 
My confusion here is that the chart needs to map to euclidean space but the quotient space is not really that. 

Why do we need the quotient space? 




Theory Background:

\begin{enumerate}
    \item Function Space
    \begin{itemize}
        \item Distance.
        \item Epsilon equivalence / equivalence.
    \end{itemize}
    \item Function space as a manifold. 
    \begin{itemize}
        \item Smooth structure on the manifold. (Should motivate the weight space).
    \end{itemize}
    \item Quotient topology on the weight space with the equivalence relation given by epsilon equivalence with epsilon set to 0. 
    \begin{itemize}
    \item Properties of the quotient space. I think we should give an example that it is not clear what it looks like and what its topological properties are. Which subsets are connected if any etc -- motivates the quotient space. 
    \end{itemize}
\end{enumerate}

Theory Algorithm:

\begin{enumerate}
    \item Basic facts about time to compute. It is quadratic in models to compare. 
    \item We will optimize by considering anchor points and this can be compressed to comparing to loss. 
    \item Should potentially lead to quasi monte carlo. (iffy about this)
\end{enumerate}

Thoughts on quasi monte carlo:
We need to be careful, it is true that we are approximating an integral, however, when we doing our speed up, we are essentially comparing a function to a "made up" function. The made up function only exists for speed up purposes and is really just another function in function space (if we are careful about well definedness). 


\section{abstract}
In this paper, we propose an efficient algorithm to visualise symmetries in parametric models. Typically the models that we use are defined w.r.t a parameter space, where non-equal parameters can produce the same function; this is the model unidentifiability problem. The method we propose allows us to identify parameters that are functionally equivalent and to visualise what the space of functions looks like when these symmetries are quotiented out. 
Specifically, we experiment on simple cases, but they identify and provide possible solutions for more complicated scenarios.
In particular we look at optimising the number of comparisons to be done using theoretical lower bounds on differences that we prove. 

\section{Introduction}



READ ASAP
\begin{itemize}
    \item https://arxiv.org/pdf/1906.06994.pdf
    \item https://www.sciencedirect.com/science/article/abs/pii/S0893608005800371
    \item http://bayesiandeeplearning.org/2017/papers/15.pdf
    \item https://www.sciencedirect.com/science/article/abs/pii/S0925231207003967
\end{itemize}





% Introduction Outline
\todo{Kate and Janith: DO THIS ASAP, you nonces}
\begin{itemize}
    \item Why is it important for a model to be identifiable?
    \begin{itemize}
        \item Bayesian paper - unidentifiability makes it difficult to learn using MCMC and VI
        \item avoid inefficient training weights due to unseen similarities/symmetries?
        \item We further enforce the importance with motivating use cases (below)...
    \end{itemize}
    
    \item There are three use cases
    \begin{enumerate}
        \item understanding of NN weight space (symmetries) \begin{itemize}
            \item general understanding
            \item visualise
            \item mathematically represent and analyse the geometry
        \end{itemize}
        \item for better optimisation [bayesian inference paper]
        \begin{itemize}
            \item improving search space
            \item characterises the existance of multiple global minimisers [uniqueness of weights]
        \end{itemize}
        \item quantifying the generalisability of the model/neighbourhoods of models for practical uses
        \begin{itemize}
            \item e.g. improved training and development of ML models in applications [flat minima] 
            \item multitask/meta learning [michilis / janith paper].
        \end{itemize}
    \end{enumerate}
    
    \item Background
    \begin{itemize}
        \item Bayesian Inference paper
        \begin{itemize}
            \item ReLU symmetries
            \item apply to MCMC and VI to get better results
            \item reparameterisation (constraints) that account for the symmetries, does not change the mappings
        \end{itemize}
        \item Uniqueness of Weights for input-output maps
        \begin{itemize}
            \item symmetries in odd functions (e.g. tanh)
            \item Specify finite group of symmetries
            \item Define Irreducibility of NN (another form of symmetries?)
        \end{itemize}
        \item Uniqueness of Weights for NN
        \begin{itemize}
            \item \todo{@Janith}
        \end{itemize}
        \item EXTRA: Uniqueness of weights in single-layer perceptrons - looks at symmetries in a different way...
        \item visualisation tools?
    \end{itemize}
    \item Summary of Work
    \begin{itemize}
        \item Visualisation tool: Mani-PEDI
        \item Given a model architecture and weight space
        \item \todo{@Janith FIX} Analyse the quotient space, where the model is identifiable, after accouting symmetries (through a functional equivalence relation)
        \item Taking its MSE loss function, visualise it (using UMAP)
        \item Show how the visualisation can be interpretted to view where and what (kind) the symmetries are
    \end{itemize}
    \item Contributions
    \begin{itemize}
        \item Visualisation tool 
        \item Optimised search for identifiability
        \item Demonstrations to applications in meta-learning/transfer learning
    \end{itemize}
    \item Paper Layout
\end{itemize}


==> reviews.tex <==
\section{Meta-Review}

1. Overall Decision
Accept
2. Please provide a brief summary of your decision
This paper proposes an algorithm to visualize the equivalence classes in the parameter space of neural networks. The reviewers raised some issues about presentation (e.g. missing abstract) and points that require clarification. This should be improved in the final version. That said, all reviewers agree that the problem of visualizing the symmetries of the parameter space is very interesting and worthy of inclusion in the workshop. I therefore recommend acceptance of this paper.


\section{Reviews}
\subsection{Review 1}
Questions
1. Please provide a summary of the work
This paper presents a tool to visualise the isotropy group of a parameter on the dataset for a neural network. They show examples of this behaviour in very small neural networks.
2. Please list the strengths of the work along the axes of technical soundness, novelty, technical execution, and experimental design (if applicable).
The work is interesting. I do not think I had ever seen any research along these lines. I cannot asses how good this work is in its context, as I have not seen anything like it before, but a priori I would be worried about its usefulness. Let $G$ be a Lie group acting faithfully on $M$. Assuming that we want to "quotient" by $G$, we are interested in performing optimisation on the space of orbits $M/G$. The present work shows how to visualise the isotropy group $G_x$. I have two main doubts about this approach:
- Why would we want to study $G_x$---\ie, the fibre of $M/G$ at one point, when we actually want to study at least the local structure of $M/G$. This gives no information in this regard.
- Why would we want to visualise it? Visualisations may help in _very_ low dimension, but this is the opposite to the setting that we are working on, that is, that of neural networks.
- We have to solve a full optimisation problem to find (an approximation of) the isotropy group at __one__ point. On the other hand, in optimisation, we want to at least understand the local geometry of our problem or, if we are going to use there results online, the method should not be slower than one forward/backward pass. Given all this, how does this method fit in the picture?

I believe that if the authors are able to answer these questions very clearly and show high dimensional examples that back their method, this could be an interesting paper, as anything that helps visualising the inner workings of a neural network can be potentially interesting.
3. Please briefly highlight the weaknesses, if any, of the current submissions and please recommend concrete suggestions for improvement.
- The paper does not have an abstract?!
- References to books. The authors cite several times Lee's book on optimisation on manifolds when talking about the isotropy group. It is good etiquette when referencing a large textbook on the subject to say at least which section one is referring to, otherwise the reference is does not serve its purpose at all.
- Line 42. "... the structure of the orbit can be non-trivial". What do the authors mean here. Is it related to principal / non-principal orbits? What does it mean for the structure of an orbit to be "non-trivial"?
- Approximation. How does this compare to the obvious solution to this problem: Find a gradient, see that the function is a submersion at that point---there exist directions on which the gradients either zero or very close to zero. Follow those directions. Of course this is notably more expensive, but I would assume that one would explore the isotropy class of the dataset much more efficiently?
Minor:
- Footnote 3. It should be $g_i \circ \dots \circ g_1$.
- The authors should consider compressing the images in the pdf, as the pdf now weights over 10MB and
5. Significance and novelty of contributions
Somewhat Novel, the contributions are interesting and would make for a solid paper if executed well
6. Presentation and Readability
Clearly Written. the paper is easy to read and follow
7. Overall score for this work.
2 (Accept)
8. Please rate your confidence level in your assessment of the overall score.
Somewhat Confident
9. Would you like to nominate this paper as a contributed talk?
No, this paper should not be considered for a contributed talk.

\subsection{Review 2}

Reviewer #6
Questions
1. Please provide a summary of the work
The authors seek to understand the symmetries of (potentially complex) neural networks - a very difficult task. Towards this end, they build a tool which helps visually and empirically explore such symmetries.
2. Please list the strengths of the work along the axes of technical soundness, novelty, technical execution, and experimental design (if applicable).
The idea to use optimization (in particular SGD) to explore symmetries is very interesting. The authors use their method to 'recover' known symmetries of a simple neural network.
3. Please briefly highlight the weaknesses, if any, of the current submissions and please recommend concrete suggestions for improvement.
The simple neural network the authors demonstrate their tool on is extremely simple, and it is not at all obvious that this tool will be effective on complex networks.

Moreover, it is not easy to read the plots their tool is outputting. Perhaps the authors could put together a comprehensive 'guide' displaying what certain symmetries will look like in their tool.

Finally, after applying a dimensionality reduction (UMAP), it seems a lot of the important features the symmetries seem to be lost (although perhaps I'm unable to effectively read the output plots of GENNI).

Nonetheless, I think this paper is worth accepting because I think the idea of visually exploring symmetries of the parameter space is a very important (and also very difficult) problem, and deserves future attention.
5. Significance and novelty of contributions
Somewhat Novel, the contributions are interesting and would make for a solid paper if executed well
6. Presentation and Readability
Minor Presentation Issues. The paper is generally well written but suffers from minor mistakes ---i.e. grammar, unclear notation, experiments etc ...
7. Overall score for this work.
3 (Strong Accept)
8. Please rate your confidence level in your assessment of the overall score.
Not Confident
9. Would you like to nominate this paper as a contributed talk?
Yes, this paper should be a contributed talk at the workshop.

\subsection{Review 3}
Reviewer #7
Questions
1. Please provide a summary of the work
This paper provides a new approach of visualising the equivalence classes of the parameters within neural networks. The approach is a simple one: use SGD to find the parameters and set the loss function as the L2-loss between the network outputs w.r.t. different parameters. The authors provide explicit visualisations on simple networks and show provide some remarks on the topology/geometry of the loss surface.
2. Please list the strengths of the work along the axes of technical soundness, novelty, technical execution, and experimental design (if applicable).
Overall, the paper is well-written and flows nicely. The perspective is interesting too; I think that it explores an interesting area (namely the equivalence classes in the parameter space of networks + the quotient space under this equivalence) which is not explored much in the deep learning community.

The proposed approach to use SGD as an approximate way to identify equivalence classes (which are often intractable otherwise) is reasonable. The authors did not provide the hyper-parameters they used for the algorithm; I am wondering are learning rates standard for example or they require quite a bit of tuning?

Also- what would be the run-time of GENNI? It is mentioned in Section 3 that a Gram-Schmidt procedure is necessary; would this be very slow in practice?
3. Please briefly highlight the weaknesses, if any, of the current submissions and please recommend concrete suggestions for improvement.
While I think the perspective is interesting, there are not too much actionable insights that can be derived from it. For example, I do not see how this would enable practitioners to easily identify regions of good weight initialisation.

Did the authors consider other types of equivalences or other types of group actions? Especially ones where there are non-trivial isotropy groups (fixed points; non-free action) and what would the implications be from the loss surface/deep learning model standpoint?
5. Significance and novelty of contributions
Somewhat Novel, the contributions are interesting and would make for a solid paper if executed well
6. Presentation and Readability
Clearly Written. the paper is easy to read and follow
7. Overall score for this work.
2 (Accept)
8. Please rate your confidence level in your assessment of the overall score.
Somewhat Confident
9. Would you like to nominate this paper as a contributed talk?
No, this paper should not be considered for a contributed talk.
